Limits on Sub-GeV Dark Matter from the PROSPECT Reactor Antineutrino Experiment

If dark matter has mass lower than around 1 GeV, it will not impart enough energy to cause detectable nuclear recoils in many direct-detection experiments. However, if dark matter is upscattered to high energy by collisions with cosmic rays, it may be detectable in both direct-detection experiments and neutrino experiments. We report the results of a dedicated search for boosted dark matter upscattered by cosmic rays using the PROSPECT reactor antineutrino experiment. We show that such a flux of upscattered dark matter would display characteristic diurnal sidereal modulation, and use this to set new experimental constraints on sub-GeV dark matter exhibiting large interaction cross-sections.

==> PROSPECT Boosted Dark Matter/AuthorListApril2021.tex <==
\affiliation{Brookhaven National Laboratory, Upton, New York, USA}
\affiliation{Department of Physics, Drexel University, Philadelphia, Pennsylvania, USA}
\affiliation{George W.\,Woodruff School of Mechanical Engineering, Georgia Institute of Technology, Atlanta, Georgia, USA}
\affiliation{Department of Physics \& Astronomy, University of Hawaii, Honolulu, Hawaii, USA}
\affiliation{Department of Physics, Illinois Institute of Technology, Chicago, Illinois, USA}
\affiliation{Nuclear and Chemical Sciences Division, Lawrence Livermore National Laboratory, Livermore, California, USA}
\affiliation{Department of Physics, Le Moyne College, Syracuse, New York, USA}
\affiliation{National Institute of Standards and Technology, Gaithersburg, Maryland, USA}
\affiliation{High Flux Isotope Reactor, Oak Ridge National Laboratory, Oak Ridge, Tennessee, USA}
\affiliation{Physics Division, Oak Ridge National Laboratory, Oak Ridge, Tennessee, USA}
\affiliation{Department of Physics, Temple University, Philadelphia, Pennsylvania, USA}
\affiliation{Department of Physics and Astronomy, University of Tennessee, Knoxville, Tennessee, USA}
\affiliation{Institute for Quantum Computing and Department of Physics and Astronomy, University of Waterloo, Waterloo, Ontario, Canada}
\affiliation{Department of Physics, University of Wisconsin, Madison, Wisconsin, USA}
\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, Connecticut, USA}
\author{M.\,Andriamirado}
\affiliation{Department of Physics, Illinois Institute of Technology, Chicago, Illinois, USA}
\author{A.\,B.\,Balantekin}
\affiliation{Department of Physics, University of Wisconsin, Madison, Wisconsin, USA}
\author{H.\,R.\,Band}
\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, Connecticut, USA}
\author{C.\,D.\,Bass}
\affiliation{Department of Physics, Le Moyne College, Syracuse, New York, USA}
\author{D.\,E.\,Bergeron}
\affiliation{National Institute of Standards and Technology, Gaithersburg, Maryland, USA}
\author{N.\,S.\,Bowden}
\affiliation{Nuclear and Chemical Sciences Division, Lawrence Livermore National Laboratory, Livermore, California, USA}
\author{C.\,D.\,Bryan}
\affiliation{High Flux Isotope Reactor, Oak Ridge National Laboratory, Oak Ridge, Tennessee, USA}
\author{T.\,Classen}
\affiliation{Nuclear and Chemical Sciences Division, Lawrence Livermore National Laboratory, Livermore, California, USA}
\author{A.\,J.\,Conant}
\affiliation{George W.\,Woodruff School of Mechanical Engineering, Georgia Institute of Technology, Atlanta, Georgia, USA}
\author{G.\,Deichert}
\affiliation{High Flux Isotope Reactor, Oak Ridge National Laboratory, Oak Ridge, Tennessee, USA}
\author{M.\,V.\,Diwan}
\affiliation{Brookhaven National Laboratory, Upton, New York, USA}
\author{M.\,J.\,Dolinski}\affiliation{Department of Physics, Drexel University, Philadelphia, Pennsylvania, USA}
\author{A.\,Erickson}
\affiliation{George W.\,Woodruff School of Mechanical Engineering, Georgia Institute of Technology, Atlanta, Georgia, USA}
\author{B.\,T.\,Foust}
\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, Connecticut, USA}
\author{J.\,K.\,Gaison}
\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, Connecticut, USA}
\author{A.\,Galindo-Uribarri}\affiliation{Physics Division, Oak Ridge National Laboratory, Oak Ridge, Tennessee, USA} \affiliation{Department of Physics and Astronomy, University of Tennessee, Knoxville, Tennessee, USA}
\author{C.\,E.\,Gilbert}\affiliation{Physics Division, Oak Ridge National Laboratory, Oak Ridge, Tennessee, USA} \affiliation{Department of Physics and Astronomy, University of Tennessee, Knoxville, Tennessee, USA}
\author{S.\,Hans}\affiliation{Brookhaven National Laboratory, Upton, New York, USA}
\author{A.\,B.\,Hansell}
\affiliation{Department of Physics, Temple University, Philadelphia, Pennsylvania, USA}
\author{K.\,M.\,Heeger}
\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, Connecticut, USA}
\author{B.\,Heffron}\affiliation{Physics Division, Oak Ridge National Laboratory, Oak Ridge, Tennessee, USA} \affiliation{Department of Physics and Astronomy, University of Tennessee, Knoxville, Tennessee, USA}
\author{D.\,E.\,Jaffe}
\affiliation{Brookhaven National Laboratory, Upton, New York, USA}
\author{S.\,Jayakumar}\affiliation{Department of Physics, Drexel University, Philadelphia, Pennsylvania, USA}
\author{X.\,Ji}
\affiliation{Brookhaven National Laboratory, Upton, New York, USA}
\author{D.\,C.\,Jones}
\affiliation{Department of Physics, Temple University, Philadelphia, Pennsylvania, USA}
\author{J. Koblanski}\affiliation{Department of Physics \& Astronomy, University of Hawaii, Honolulu, Hawaii, USA}
\author{O.\,Kyzylova}\affiliation{Department of Physics, Drexel University, Philadelphia, Pennsylvania, USA}
\author{C.\,E.\,Lane}\affiliation{Department of Physics, Drexel University, Philadelphia, Pennsylvania, USA}
\author{T.\,J.\,Langford}
\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, Connecticut, USA}
\author{J.\,LaRosa}
\affiliation{National Institute of Standards and Technology, Gaithersburg, Maryland, USA}
\author{B.\,R.\,Littlejohn}
\affiliation{Department of Physics, Illinois Institute of Technology, Chicago, Illinois, USA}
\author{X.\,Lu}\affiliation{Physics Division, Oak Ridge National Laboratory, Oak Ridge, Tennessee, USA} \affiliation{Department of Physics and Astronomy, University of Tennessee, Knoxville, Tennessee, USA}
\author{J.\,Maricic}\affiliation{Department of Physics \& Astronomy, University of Hawaii, Honolulu, Hawaii, USA}
\author{M.\,P.\,Mendenhall}\affiliation{Nuclear and Chemical Sciences Division, Lawrence Livermore National Laboratory, Livermore, California, USA}
\author{A.\,M.\,Meyer}\affiliation{Department of Physics \& Astronomy, University of Hawaii, Honolulu, Hawaii, USA}
\author{R.\,Milincic}\affiliation{Department of Physics \& Astronomy, University of Hawaii, Honolulu, Hawaii, USA}
\author{P.\,E.\,Mueller}\affiliation{Physics Division, Oak Ridge National Laboratory, Oak Ridge, Tennessee, USA} 
\author{H.\,P.\,Mumm}
\affiliation{National Institute of Standards and Technology, Gaithersburg, Maryland, USA}
\author{J.\,Napolitano}
\affiliation{Department of Physics, Temple University, Philadelphia, Pennsylvania, USA}
\author{R.\,Neilson}\affiliation{Department of Physics, Drexel University, Philadelphia, Pennsylvania, USA}
\author{J.\,A.\,Nikkel}
\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, Connecticut, USA}
\author{S.\,Nour}
\affiliation{National Institute of Standards and Technology, Gaithersburg, Maryland, USA}
\author{J.\,L.\,Palomino}
\affiliation{Department of Physics, Illinois Institute of Technology, Chicago, Illinois, USA}
\author{D.\,A.\,Pushin}\affiliation{Institute for Quantum Computing and Department of Physics and Astronomy, University of Waterloo, Waterloo, Ontario, Canada}
\author{X.\,Qian}
\affiliation{Brookhaven National Laboratory, Upton, New York, USA}
\author{R.\,Rosero}
\affiliation{Brookhaven National Laboratory, Upton, New York, USA}
\author{P.\,T.\,Surukuchi}
\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, Connecticut, USA}
\author{M.\,A.\,Tyra}
\affiliation{National Institute of Standards and Technology, Gaithersburg, Maryland, USA}
\author{R.\,L.\,Varner}\affiliation{Physics Division, Oak Ridge National Laboratory, Oak Ridge, Tennessee, USA} 
\author{D.\,Venegas-Vargas}\affiliation{Physics Division, Oak Ridge National Laboratory, Oak Ridge, Tennessee, USA} \affiliation{Department of Physics and Astronomy, University of Tennessee, Knoxville, Tennessee, USA}
\author{P.\,B.\,Weatherly}\affiliation{Department of Physics, Drexel University, Philadelphia, Pennsylvania, USA}
\author{C.\,White}
\affiliation{Department of Physics, Illinois Institute of Technology, Chicago, Illinois, USA}
\author{J.\,Wilhelmi}
\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, Connecticut, USA}
\author{A.\,Woolverton}\affiliation{Institute for Quantum Computing and Department of Physics and Astronomy, University of Waterloo, Waterloo, Ontario, Canada}
\author{M.\,Yeh}
\affiliation{Brookhaven National Laboratory, Upton, New York, USA}
\author{C.\,Zhang}
\affiliation{Brookhaven National Laboratory, Upton, New York, USA}
\author{X.\,Zhang}
\affiliation{Nuclear and Chemical Sciences Division, Lawrence Livermore National Laboratory, Livermore, California, USA}


